Measurement of the Higgs boson coupling properties in the $H\rightarrow ZZ^{*} \rightarrow 4\ell$ decay channel at $\sqrt{s}$ = 13 TeV with the ATLAS detector

The coupling properties of the Higgs boson are studied in the four-lepton decay channel using 36.1 fb$^{-1}$ of $pp$ collision data from the LHC at a centre-of-mass energy of 13 TeV collected by the ATLAS detector. Cross sections are measured for the four key production modes in several exclusive regions of the Higgs boson production phase space and are interpreted in terms of coupling modifiers. The inclusive cross section times branching ratio for $H \rightarrow ZZ^*$ decay and for a Higgs boson absolute rapidity below 2.5 is measured to be $1.73^{+0.24}_{-0.23}$(stat.)$^{+0.10}_{-0.08}$(exp.)$\pm 0.04$(th.) pb compared to the Standard Model prediction of $1.34\pm0.09$ pb. In addition, the tensor structure of the Higgs boson couplings is studied using an effective Lagrangian approach for the description of interactions beyond the Standard Model. Constraints are placed on the non-Standard-Model CP-even and CP-odd couplings to $Z$ bosons and on the CP-odd coupling to gluons.

==> sec_auxiliary.tex <==
\label{sec:Auxiliary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% m4l PLOTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[!htbp]
 \centering 
  \subfloat[\label{fig:finalMassesSignalch0}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/m4lCons_4mu}}
  \subfloat[\label{fig:finalMassesSignalch1}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/m4lCons_2mu2e}}\\
  \subfloat[\label{fig:finalMassesSignalch3}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/m4lCons_2e2mu}}
  \subfloat[\label{fig:finalMassesSignalch2}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/m4lCons_4e}}
  %% \subfloat[\label{fig:finalMassesSignalch0}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/m4lCons_4mu_prelim}}
  %% \subfloat[\label{fig:finalMassesSignalch1}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/m4lCons_2mu2e_prelim}}\\
  %% \subfloat[\label{fig:finalMassesSignalch3}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/m4lCons_2e2mu_prelim}}
  %% \subfloat[\label{fig:finalMassesSignalch2}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/m4lCons_4e_prelim}}
  \caption{The observed and expected four-lepton invariant mass distribution for the selected Higgs boson candidates with a constrained $Z$ boson mass, shown for an integrated luminosity of \Lum at $\sqrt{\mathrm{s}}=$~13~TeV for the  different channels of the analysis: (a)~$4\mu$, (b)~$2\mu2e$, (c)~$2e2\mu$ and (d)~$4e$. The error bars represent 68.3\% central confidence interval statistical uncertainty. The systematic uncertainty on the prediction is shown by the dashed band. %\label{fig:finalMassesSignalch}
  }
   
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CATEGORIZATION OBSERVABLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=0.4\textwidth]{figures/auxiliary/Inc_NJets_4l}
%\includegraphics[width=0.4\textwidth]{figures/auxiliary/Jet1_pt4l_4l}
%\includegraphics[width=0.4\textwidth]{figures/auxiliary/Jet2_mJJ_4l}
%\includegraphics[width=0.4\textwidth]{figures/auxiliary/Jet2_VBF_Leadjet_pt_4l}
%\includegraphics[width=0.4\textwidth]{figures/auxiliary/Jet2_VH_pt4l_4l}
%\end{center}
%\caption{The observed and expected distributions of $N_{jet}$, \pt$_{4l}$ in 1 jet category, $m_{jj}$ in 2 jet category, \pt$_{j1}$ in VBF-enriched category and \pt$_{4l}$ in VH-enriched category for an integrated luminosity of \Lum collected at $\sqrt{s}=$~13~TeV.  Error bars represent 68.3\% central confidence intervals.}
%\label{fig:categoryVars}
%\end{figure}
\clearpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ACCEPTANCE PLOTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!htbp]	
\centering
\includegraphics[width=0.95\linewidth]{figures/auxiliary/combinedAcc_Stage0}
\caption{Signal acceptance obtained as the ratio of the number of simulated signal events satisfying the event selection criteria in each reconstructed event category to the total number of events generated in the phase space specified by a given Stage-0 production bin. }
 \label{fig:STXS_redStage0_acc}
\end{figure}

\begin{figure}[!htbp]	
\centering
\includegraphics[width=0.95\linewidth]{figures/auxiliary/combinedAcc}
\caption{Signal acceptance obtained as the ratio of the number of simulated signal events satisfying the event selection criteria in each reconstructed event category to the total number of events generated in the phase space specified by a given reduced Stage-1 production bin. }
 \label{fig:STXS_redStage1_acc}
\end{figure}

\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ACCEPTANCE TABLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[htbb!]
  \centering 
%  \scriptsize
  \caption{Signal acceptance obtained as the ratio of the number of simulated signal events satisfying the event selection criteria in each reconstructed event category over the total number of events generated in the phase space specified by a given reduced Stage-1 \ggF production bin.  Results are obtained in bins of \BDT discriminants using coarse binning with several bins merged into one. The symbol $-$ represents the cases in which the acceptance is $<0.01\%$. 
  }
  \label{tab:NsAeggF}
  \vspace{0.1cm}
  \setlength{\tabcolsep}{1cm}
  {\renewcommand{\arraystretch}{1.1}%
    
    \resizebox{\linewidth}{!}{

  
  \begin{tabular}{* {1} {@{\hspace{2pt}}l@{\hspace{2pt}}}* {5} {@{\hspace{2pt}}c@{\hspace{2pt}}}}
      \hline\hline
    %\noalign{\vspace{0.05cm}}
    Category    & 
    \STXSggFZeroJ  & 
    \STXSggFOneJL  & 
    \STXSggFOneJM & 
    \STXSggFOneJH & \STXSggFTwoJ\\ \hline  
                 
\CatZeroJ, \BDT Bin 0-4               & $0.038 \pm 0.004 $ & $0.0028 \pm 0.0009 $ & $ - $ & $ - $ & $ - $\\
\CatZeroJ, \BDT Bin 5-9               & $0.085 \pm 0.008 $ & $0.013 \pm 0.004 $ & $0.0023 \pm 0.0007 $ & $ - $ & $ - $\\
\CatZeroJ, \BDT Bin 10-14             & $0.077 \pm 0.008 $ & $0.024 \pm 0.007 $ & $0.0093 \pm 0.0028 $ & $0.0018 \pm 0.0005 $ & $0.0019 \pm 0.0009 $\\
\CatOneJL, \BDT Bin 0-4               & $0.018 \pm 0.006 $ & $0.101 \pm 0.016 $ & $0.0032 \pm 0.0006 $ & $ - $ & $0.0058 \pm 0.0018 $\\
\CatOneJL, \BDT Bin 5-9               & $0.0053 \pm 0.0017 $ & $0.062 \pm 0.011 $ & $0.0034 \pm 0.0006 $ & $ - $ & $0.0055 \pm 0.0017 $\\
\CatOneJM, \BDT Bin 0-4               & $ - $ & $0.0019 \pm 0.0004 $ & $0.129 \pm 0.022 $ & $0.0042 \pm 0.0010 $ & $0.011 \pm 0.004 $\\
\CatOneJM, \BDT Bin 5-9               & $ - $ & $ - $ & $0.063 \pm 0.010 $ & $0.0056 \pm 0.0012 $ & $0.0052 \pm 0.0018 $\\
\CatOneJH                           & $ - $ & $ - $ & $ - $ & $0.24 \pm 0.05 $ & $0.0062 \pm 0.0022 $\\
\CatVBFLow, \BDT Bin 0-4              & $0.0016 \pm 0.0008 $ & $0.010 \pm 0.004 $ & $0.014 \pm 0.005 $ & $0.019 \pm 0.007 $ & $0.094 \pm 0.019 $\\
\CatVBFLow, \BDT Bin 5-9              & $ - $ & $0.0017 \pm 0.0008 $ & $0.0036 \pm 0.0015 $ & $0.0075 \pm 0.0030 $ & $0.030 \pm 0.008 $\\
\CatVBFHigh                         & $ - $ & $ - $ & $ - $ & $0.0060 \pm 0.0027 $ & $0.013 \pm 0.004 $\\
\CatVHHad, \BDT Bin 0-4               & $0.0015 \pm 0.0011 $ & $0.0079 \pm 0.0033 $ & $0.016 \pm 0.005 $ & $0.017 \pm 0.007 $ & $0.052 \pm 0.013 $\\
\CatVHHad, \BDT Bin 5-9               & $ - $ & $0.0021 \pm 0.0008 $ & $0.0030 \pm 0.0010 $ & $0.0049 \pm 0.0018 $ & $0.025 \pm 0.006 $\\
\CatVHLep                           & $ - $ & $ - $ & $ - $ & $ - $ & $ - $\\
\CatttH                             & $ - $ & $ - $ & $ - $ & $ - $ & $0.0021 \pm 0.0007 $\\
Combined                            & $0.228 \pm 0.019 $ & $0.228 \pm 0.034 $ & $0.25 \pm 0.04 $ & $0.30 \pm 0.06 $ & $0.25 \pm 0.06 $\\

                   \hline\hline
    \end{tabular}
}}
\end{table*}




\begin{table*}[htbb!]
  \centering 
%  \scriptsize
  \caption{Signal acceptance obtained as the ratio of the number of simulated signal events satisfying the event selection criteria in each reconstructed event category over the total number of events generated in the phase space specified by the given reduced Stage-1 \VBF and \VH production bins. Results are obtained in bins of \BDT discriminants using coarse binning with several bins merged into one. The symbol $-$ represents the cases in which the acceptance is $<0.01\%$. 
}
  \label{tab:NsAeVBFVH}
  
    \vspace{0.1cm}
  \setlength{\tabcolsep}{1cm}
  {\renewcommand{\arraystretch}{1.1}%
    
    \resizebox{\linewidth}{!}{

  
  \begin{tabular}{* {1} {@{\hspace{2pt}}l@{\hspace{2pt}}}* {5} {@{\hspace{2pt}}c@{\hspace{2pt}}}}
      \hline\hline
    \noalign{\vspace{0.05cm}}
    Category    & 
     \STXSVBFLow & 
     \STXSVBFHigh & 
    \STXSVHHad & 
     \STXSVHLep \\ 
     
     \hline               
\CatZeroJ, \BDT Bin 0-4               & $0.00186 \pm 0.00030 $ & $ - $ & $0.00134 \pm 0.00033 $ & $0.0036 \pm 0.00097 $\\
\CatZeroJ, \BDT Bin 5-9               & $0.0067 \pm 0.0013 $ & $ - $ & $0.0045 \pm 0.0009 $ & $0.0136 \pm 0.0017 $\\
\CatZeroJ, \BDT Bin 10-14             & $0.0107 \pm 0.0029 $ & $ - $ & $0.0076 \pm 0.0018 $ & $0.044 \pm 0.005 $\\
\CatOneJL, \BDT Bin 0-4               & $0.0131 \pm 0.0011 $ & $ - $ & $0.0213 \pm 0.0026 $ & $0.0084 \pm 0.0009 $\\
\CatOneJL, \BDT Bin 5-9               & $0.0211 \pm 0.0013 $ & $ - $ & $0.0101 \pm 0.0011 $ & $0.0049 \pm 0.0005 $\\
\CatOneJM, \BDT Bin 0-4               & $0.0148 \pm 0.0025 $ & $ - $ & $0.0250 \pm 0.0034 $ & $0.0122 \pm 0.0011 $\\
\CatOneJM, \BDT Bin 5-9               & $0.0280 \pm 0.0029 $ & $ - $ & $0.0054 \pm 0.0007 $ & $0.0038 \pm 0.0004 $\\
\CatOneJH                           & $0.0149 \pm 0.0021 $ & $0.070 \pm 0.009 $ & $0.0099 \pm 0.0012 $ & $0.0124 \pm 0.0009 $\\
\CatVBFLow, \BDT Bin 0-4              & $0.0346 \pm 0.0033 $ & $0.005 \pm 0.005 $ & $0.036 \pm 0.004 $ & $0.0120 \pm 0.0016 $\\
\CatVBFLow, \BDT Bin 5-9              & $0.099 \pm 0.0097 $ & $0.015 \pm 0.016 $ & $0.0036 \pm 0.0006 $ & $ - $\\
\CatVBFHigh                         & $0.0011 \pm 0.0004 $ & $0.234 \pm 0.018 $ & $0.0066 \pm 0.0007 $ & $0.00198 \pm 0.00031 $\\
\CatVHHad, \BDT Bin 0-4               & $0.0110 \pm 0.0013 $ & $0.0062 \pm 0.0006 $ & $0.0198 \pm 0.0023 $ & $0.0052 \pm 0.0007 $\\
\CatVHHad, \BDT Bin 5-9               & $0.0029 \pm 0.0006 $ & $0.0030 \pm 0.0004 $ & $0.071 \pm 0.007 $ & $0.0046 \pm 0.0005 $\\
\CatVHLep                           & $ - $ & $ - $ & $ - $ & $0.092 \pm 0.008 $\\
\CatttH                             & $ - $ & $0.0022 \pm 0.0004 $ & $0.0024 \pm 0.0005 $ & $ - $\\
Combined                            & $0.261 \pm 0.014 $ & $0.336 \pm 0.029 $ & $0.224 \pm 0.019 $ & $0.221 \pm 0.018 $\\

                   \hline\hline
    \end{tabular}
}}
\end{table*}


\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%CORRELATION MATRICES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure}[!htbp]
    \centering
    \subfloat[Stage 0, expected]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/corr_mu}}
    \subfloat[Reduced Stage 1, expected]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/corr_muRedStage1}} \\
    \subfloat[Stage 0, observed]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/data_mu}}
    \subfloat[Reduced Stage 1, observed]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/data_muRedStage1}} 
    \caption{Correlation matrix for the different parameters of interest when fitting the Asimov dataset  for (a) Stage-0 and (b) reduced Stage-1 signal strength parameters and when fitting the data for (c) Stage-0 and (d) reduced Stage-1.}
    \label{fig:ObservedCorr}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%COVARIANCE MATRICES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!htbp]
    \centering
\subfloat[Stage 0, expected]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/Cov_mu}}
\subfloat[Reduced Stage 1, expected]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/Cov_muRedStage1}}\\
\subfloat[Stage 0, observed]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/Cov_data_mu}}
\subfloat[Reduced Stage 1, observed]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/Cov_data_muRedStage1}}
    \caption{Covariance matrix for the different parameters of interest when fitting the Asimov dataset for (a) Stage-0 and (b) reduced Stage-1 signal strength parameters and when fitting the data for (c) Stage-0 and (d)  reduced Stage-1.}
\label{fig:Covariance}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NLL SCANS STXS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% \begin{figure}[!htbp]
%%        \centering
%%	
%%	        \subfloat[]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/XS}} 
%%	        \subfloat[]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/mu}}
%%	        \caption{Negative log-likelihood scans with and without systematics for expected and observed data for the inclusive measurement of (a) $\sigma \cdot \mbr(H\to ZZ^*)$ and (b) signal strength $\mu$.}
%%        \label{fig:STXS_incl}
%%	    \end{figure}
%%

	\begin{figure}[!htbp]
	    \centering
	    \subfloat[$\sigma_{\textrm{ggF}}\cdot B$]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/XS_gg2H}}
	    \subfloat[$\sigma_{\textrm{VBF}}\cdot B$]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/XS_VBF}} \\
%	    \subfloat[$ \sigma_{VH} $]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/XS_VH}}
%	    \subfloat[$ \sigma_{ttH}$]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/XS_ttH}}
	    \caption{Observed (black line) and SM expected (blue line) negative log-likelihood scans with (solid line) and without (dashed line) systematics for the \sBRZZ measurement in Stage-0 production bins.  Negative log-likelihood scans are not reported for $ \sigma_{\VH} $ and $ \sigma_{\ttH}$ where the limits are derived using pseudo-experiments.}
	    \label{fig:NLLXSpoiStage0}
	\end{figure}


	\begin{figure}[!htbp]
	    \centering
	    \subfloat[$ \mu_{\textrm{ggF}}$]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/mu_gg2H}}
	    \subfloat[$ \mu_{\textrm{VBF}}$]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/mu_VBF}} \\
%	    \subfloat[$ \mu_{VH} $]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/mu_VH}}
%	    \subfloat[$ \mu_{ttH}$]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/mu_ttH}}
	    \caption{Observed (black line) and SM expected (blue line) negative log-likelihood scans with (solid line) and without (dashed line) systematics for the signal strength  measurement in Stage-0 production bins. Negative log-likelihood scans are not reported for $ \mu_{\VH} $ and $ \mu_{\ttH}$ where the limits are derived using pseudo-experiments.}
	    \label{fig:NLLMupoiStage0}
	\end{figure}


\begin{figure}[!htbp]
 \centering
\subfloat[$\sigma_{\emph{\STXSggFZeroJ}}\cdot B$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/XS_gg2H_0J}}
\subfloat[$\sigma_{\emph{\STXSggFOneJL}}\cdot B$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/XS_gg2H_1J_PTH_0_60}}  \subfloat[$\sigma_{\emph{\STXSggFOneJM}}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/XS_gg2H_1J_PTH_60_120}} \\
\subfloat[$ \sigma_{\emph{\STXSggFOneJH}}\cdot B$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/XS_gg2H_1J_PTH_GT120}}
\subfloat[$ \sigma_{\emph{\STXSggFTwoJ}}\cdot B$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/XS_gg2H_GE2J}}
%  \subfloat[$ \sigma_{ttH}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/XS_ttH_all}} \\
\subfloat[$\sigma_{\emph{\STXSVBFLow}}\cdot B$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/XS_VBF_qq2qq_PTJET1_GT200}}\\
  \subfloat[$\sigma_{\emph{\STXSVBFHigh}}\cdot B$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/XS_VBF_qq2qq_PTJET1_LE200}} 
%  \subfloat[$\sigma_{VH^{Had}}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/XS_VH_Had}} \\
%  \subfloat[$\sigma_{VH^{Lep}}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/XS_VH_Lep}}
 \caption{Observed (black line) and SM expected (blue line) negative log-likelihood scans with (solid line) and without (dashed line) systematics for the \sBRZZ  measurement in reduced Stage-1 production bins. Negative log-likelihood scans are not reported for $\sigma_{\emph{\STXSVHHad}}$, $\sigma_{\emph{\STXSVHLep}}$ and $\sigma_{\emph{\STXSttH}}$ where the limits are derived using pseudo-experiments.}
 \label{fig:NLLXSpoiRedStage1}
\end{figure}


\begin{figure}[!htbp]
 \centering
\subfloat[$ \mu_{\emph{\STXSggFZeroJ}}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/mu_gg2H_0J}}
  \subfloat[$\mu_{\emph{\STXSggFOneJL}}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/mu_gg2H_1J_PTH_0_60}} 
  \subfloat[$ \mu_{\emph{\STXSggFOneJM}}$] {\includegraphics[width=0.3\linewidth]{figures/auxiliary/mu_gg2H_1J_PTH_60_120}} \\
  \subfloat[$ \mu_{\emph{\STXSggFOneJH}}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/mu_gg2H_1J_PTH_GT120}}
  \subfloat[$ \mu_{\emph{\STXSggFTwoJ}}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/mu_gg2H_GE2J}}
%  \subfloat[$ \mu_{ttH}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/mu_ttH_all}} \\
  \subfloat[$\mu_{\emph{\STXSVBFLow}}$ ] {\includegraphics[width=0.3\linewidth]{figures/auxiliary/mu_VBF_qq2qq_PTJET1_GT200}}\\
  \subfloat[$\mu_{\emph{\STXSVBFHigh}}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/mu_VBF_qq2qq_PTJET1_LE200}} 
%  \subfloat[$\mu_{VH^{Had}}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/mu_VH_Had}} \\
%  \subfloat[$\mu_{VH^{Lep}}$]{\includegraphics[width=0.3\linewidth]{figures/auxiliary/mu_VH_Lep}}
 \caption{Observed (black line) and SM expected (blue line) negative log-likelihood scans with (solid line) and without (dashed line) systematics for the measurement of the signal strength $\mu$ in reduced Stage-1 production bins. Negative log-likelihood scans are not reported for $\mu_{\emph{\STXSVHHad}}$, $\mu_{\emph{\STXSVHLep}}$ and $\mu_{\emph{\STXSttH}}$ where the limits are derived using pseudo-experiments.}
 \label{fig:NLLMupoiRedStage1}
\end{figure}




\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mu values for each production bin
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[!htbp]
  \def\arraystretch{1.1}
  \centering
  \caption{The signal strengths $\mu$ for the inclusive production and 
  in each Stage-0 and reduced Stage-1 production bin for an integrated luminosity of \Lum and at $\sqrt{\mathrm{s}}=13$~\TeV. The \bbH contribution is considered as a part of the  \ggF production bins.
    The upper limits correspond to the 95\%~CL obtained with pseudo-experiments using the  CL$_{\textrm s}$  method. The uncertainties are given as (stat.)+(syst.).  
  }
  \label{tab:Stage01_aux}
  \label{tab:XS_cat_result_aux}  

   
     \vspace{0.1cm}
  %\setlength{\tabcolsep}{1cm}
  {\renewcommand{\arraystretch}{1.5}
  \resizebox{0.6\linewidth}{!}{

  \begin{tabular}{l |c }
    \hline\hline
   Production bin &   Observed signal strength, $\mu$\\
    % &  \multicolumn{1}{c}{Observed}   \\
    \hline
    \multicolumn{2}{l}{Inclusive production, $|y_{H}|<2.5$}\\
    \hline
                        & 
   $1.28^{+0.18}_{-0.17}$$^{+0.08}_{-0.06}$$^{+0.08}_{-0.06}$
    \\

    \hline
    \multicolumn{2}{l}{Stage-0 production bins, $|y_{H}|<2.5$}\\
    \hline
    \STXSggF                    & 
   $1.11^{+0.22}_{-0.20}$$^{+0.08}_{-0.06}$$^{+0.08}_{-0.06}$
    \\
      
    \STXSVBF                    & 
   $4.0^{+1.7}_{-1.4}$$^{+0.4}_{-0.3}$$\pm 0.4$
    \\
    
    \STXSVH                     & 
   $<3.8                  $
    \\
    
    \STXSttH                    & 
   $<7.7                  $
    \\
    
    \hline
    %\hline
    \multicolumn{2}{l}{Reduced Stage-1 production bins, $|y_{H}|<2.5$}\\
    \hline
    
    \STXSggFZeroJ               & 
    $1.22^{+0.30}_{-0.27}$$^{+0.16}_{-0.11}$
    \\
    
    \STXSggFOneJL               & 
    $0.5^{+0.8}_{-0.7}$$\pm 0.3$
    \\
    
    \STXSggFOneJM               & 
    $1.3^{+0.9}_{-0.7}$$^{+0.4}_{-0.2}$
    \\
    
    \STXSggFOneJH               & 
    $1.3^{+2.3}_{-1.7}$$^{+0.8}_{-0.3}$
    \\
    
    \STXSggFTwoJ                & 
    $1.5^{+1.2}_{-1.0}$$^{+0.7}_{-0.2}$
    \\
    
    \STXSVBFLow                 & 
$2.9^{+2.0}_{-1.6}$$^{+0.4}_{-0.3}$
\\
    
    \STXSVBFHigh                & 
$13^{+12}_{-8}$$\pm 1$
    \\
    
    \STXSVHHad                  & 
$<5.6                  $
    \\
    
    \STXSVHLep                  & 
$<9.5                  $
    \\
    
    \STXSttH                    & 
$<6.9                  $
    \\
    
    \hline\hline
  \end{tabular}
  }}
  \end{table*}

\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NLL SCANS TENSOR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 \begin{figure}[!htbp]
  \centering
  \subfloat[\label{fig:kHVVFloat}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/KHVV_KSM_float_obs}}    
  \subfloat[\label{fig:kAVVFloat}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/KAVV_KSM_float_obs}}\\
  %\subfloat[\label{fig:kHVVAVV}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/2D_36_5_KSM_float_Cat_Coupling_obs.pdf}}
   \caption{Observed (solid black line) and SM expected (dashed blue line) negative log-likelihood scans for (a) \kHVV and (b) \kAVV coupling parameters with \kSM as a free parameter of the fit, using \Lum of data at $\sqrt{\mathrm{s}}=$~13~TeV. 
    \label{fig:kBSM_1D} }
\end{figure}


 \begin{figure}[!htbp]
  \centering
\subfloat[\label{fig:kHVVkSM}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/2D_36_5_KHZZ_KSM_Cat_Coupling_obs}}
\subfloat[\label{fig:kAVVkSM}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/2D_36_5_KAZZ_KSM_Cat_Coupling_obs}}
   \caption{Observed (black line) and SM expected (blue line) two-dimensional negative log-likelihood scans for (a) \kHVV versus \kSM and (b) \kAVV versus \kSM coupling parameters using \Lum of data at $\sqrt{\mathrm{s}}=$~13~TeV. The $95\%$~CL exclusion limits are shown.}
    \label{fig:kBSM_2D} 
\end{figure}


 \begin{figure}[!htbp]
  \centering
  \subfloat[\label{fig:kAggSX0}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/kAgg_SX0}}
  \subfloat[\label{fig:kAggSX0chi}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/kAgg_SX0_chi}}
  %% \subfloat[\label{fig:kAggSX0}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/kAgg_SX0_prelim}}
  %% \subfloat[\label{fig:kAggSX0chi}]{\includegraphics[width=0.5\linewidth]{figures/auxiliary/kAgg_SX0_chi_prelim}}
   \caption{Observed (black line) and SM expected (blue line) negative log-likelihood
(a) and $\Delta\chi^2$ (b) scans for the \kAgg interpretation using Stage-0 results.  Negative log-likelihood scan is performed by parameterizing cross-section as function of \kAgg in the fit model, while  $\Delta\chi^2$  is obtained using the observed results and covariance matrix. }
    \label{fig:kAggSX} 
\end{figure}


\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BSM signal yields and acceptances
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%



\begin{table*}[!htbp]
  \def\arraystretch{1.8}
  \centering
  \caption{Signal acceptance (in percent) obtained as the ratio of the number of simulated signal events satisfying the event selection criteria in each reconstructed event category to the total number of generated events, as predicted by the \progname{MadGraph5\_aMC@NLO} generator assuming the SM coupling tensor structure or the BSM tensor structure with (\kSM = 1, | \kAVV | $\neq$ 0). 
  }
  \label{tab:BSMacceptance}

   
     \vspace{0.1cm}
  %\setlength{\tabcolsep}{1cm}
  {\renewcommand{\arraystretch}{1.5}
  \resizebox{\linewidth}{!}{


\begin{tabular}{l|cc|cc|cc}

\hline\hline
  Reconstructed & \multicolumn{2}{c|}{\ggF} &  
 \multicolumn{2}{c|}{\VBF+\STXSVHHad}  & 
 \multicolumn{2}{c}{\STXSVHLep}\\
 
 event category & SM  &  (\kSM=1, |\kAVV|=6)  & SM &  (\kSM=1, |\kAVV|=5)  & SM &  (\kSM=1, |\kAVV|=5)|  \\

%   & 344158 & 344163 & 343247 & 343253 & 344135 & 344141 \\     

\hline 


%after event selection & 23.5 $\pm$ 0.19 & 23.76 $\pm$ 0.19 & 25.13 $\pm$ 0.1 & 26.76 $\pm$ 0.14 & 26.31 $\pm$ 0.25 & 28.38 $\pm$ 0.19 \\ 

%$m_{4\ell}$-cut & 21.46 $\pm$ 0.18 & 21.70 $\pm$ 0.18 & 22.99 $\pm$ 0.1 & 24.54 $\pm$ 0.13 & 16.47 $\pm$ 0.2 & 19.45 $\pm$ 0.15 \\ 

\CatZeroJ & 11.23 $\pm$ 0.11 & 11.34 $\pm$ 0.11 & 1.36 $\pm$ 0.02 & 0.63 $\pm$ 0.02 & 5.28 $\pm$ 0.12 & 4.81 $\pm$ 0.07 \\ 

\CatOneJL & 3.78 $\pm$ 0.08 & 3.55 $\pm$ 0.08 & 2.67 $\pm$ 0.03 & 1.36 $\pm$ 0.03 & 1.12 $\pm$ 0.05 & 0.60 $\pm$ 0.03 \\ 

\CatOneJM & 2.08 $\pm$ 0.06 & 2.19 $\pm$ 0.06 & 2.88 $\pm$ 0.03 & 1.92 $\pm$ 0.04 & 1.35 $\pm$ 0.05 & 1.14 $\pm$ 0.04 \\ 

\CatOneJH & 0.62 $\pm$ 0.03 & 0.62 $\pm$ 0.03 & 1.06 $\pm$ 0.02 & 2.12 $\pm$ 0.04 & 1.11 $\pm$ 0.05 & 2.76 $\pm$ 0.06 \\ 

\CatVBFLow & 2.10 $\pm$ 0.07 & 2.18 $\pm$ 0.07 & 10.87 $\pm$ 0.07 & 7.80 $\pm$ 0.08 & 1.05 $\pm$ 0.05 & 1.42 $\pm$ 0.04 \\ 

\CatVBFHigh & 0.22 $\pm$ 0.03 & 0.30 $\pm$ 0.03 & 1.15 $\pm$ 0.02 & 5.11 $\pm$ 0.06 & 0.11 $\pm$ 0.01 & 0.32 $\pm$ 0.02 \\ 

\CatVHHadLow & 1.08 $\pm$ 0.05 & 1.21 $\pm$ 0.05 & 2.16 $\pm$ 0.03 & 2.37 $\pm$ 0.04 & 0.54 $\pm$ 0.03 & 0.41 $\pm$ 0.02 \\ 

\CatVHHadHigh & 0.32 $\pm$ 0.03 & 0.26 $\pm$ 0.02 & 0.75 $\pm$ 0.02 & 3.01 $\pm$ 0.05 & 0.22 $\pm$ 0.03 & 0.49 $\pm$ 0.02 \\ 

\CatVHLep & 0.0 $\pm$ 0.0 & 0.01 $\pm$ 0.0 & 0.02 $\pm$ 0.0 & 0.03 $\pm$ 0.0 & 5.67 $\pm$ 0.12 & 7.46 $\pm$ 0.09 \\ 

\CatttH & 0.04 $\pm$ 0.01 & 0.03 $\pm$ 0.01 & 0.07 $\pm$ 0.01 & 0.19 $\pm$ 0.01 & 0.03 $\pm$ 0.02 & 0.04 $\pm$ 0.01 \\ 

\hline\hline

\end{tabular}
}}
\end{table*}


%%Table nExp ggF 
%  \begin{table}[h!]
%\tiny\centering
%\resizebox{\linewidth}{!}{

\begin{table*}[!htbp]
  \def\arraystretch{1.8}
  \centering
  \caption{Number of expected \ggF Higgs boson events %and the corresponding signal acceptance ($\mathcal{A}$) 
  for an integrated luminosity of \Lum and at $\sqrt{\mathrm{s}}=13$~\TeV, as predicted by the \progname{MadGraph5\_aMC@NLO} generator assuming the SM coupling tensor structure or the BSM tensor structure with (\kSM = 1, | \kAVV | = 6). 
  %The signal acceptance is obtained as the ratio of the number of simulated signal events satisfying the event selection criteria in each reconstructed category over the total number of generated events. 
  The highest-order SM predicition for the sum of the \ggF, \ttH and \bbH contributions is also shown for comparison.  }
  \label{tab:BSMyields_ggF}

   
     \vspace{0.1cm}
  %\setlength{\tabcolsep}{1cm}
  {\renewcommand{\arraystretch}{1.5}
  \resizebox{\linewidth}{!}{


\begin{tabular}{l|c|c|c}

\hline\hline

 Reconstructed & Highest-order &   \progname{MadGraph5\_aMC@NLO} &  \progname{MadGraph5\_aMC@NLO}\\
 event category & SM prediction &  \ggF & \ggF  \\ 

  & \ggF+\ttH+\bbH&  (SM) & (\kSM = 1, | \kAVV | = 6)  \\ \hline 
  
%$m_{4\ell}$-cut 	& 47.47 & 31.81 & 32.84 \\


\CatZeroJ	& 26.22 & 16.64 & 17.16 \\

\CatOneJL 	& 8.09 & 5.59 & 5.38 \\

\CatOneJM       & 4.53 & 3.09 & 3.32 \\
	
\CatOneJH       & 1.11 & 0.92 & 0.95\\

\CatVBFLow      & 3.99 & 3.11 & 3.31 \\

\CatVBFHigh	& 0.34 & 0.33 & 0.45\\

\CatVHHadLow    & 2.35 & 1.60 & 1.83 \\
	
\CatVHHadHigh   & 0.43 & 0.47 & 0.40\\ 

\CatVHLep 	& 0.05 & 0.01 & 0.01 \\

\CatttH 	& 0.36 & 0.05 & 0.05\\
\hline
\hline
\end{tabular}
}}
\end{table*}


 
 
\begin{table*}[!htbp]
  \def\arraystretch{1.8}
  \centering
  \caption{Number of expected \VBF and \VH Higgs boson events %and the corresponding signal acceptance ($\mathcal{A}$) 
  for an integrated luminosity of \Lum and at $\sqrt{\mathrm{s}}=13$~\TeV, as predicted by the \progname{MadGraph5\_aMC@NLO} generator assuming the SM coupling tensor structure or the BSM tensor structure with (\kSM = 1, | \kAVV | = 5). 
  %The signal acceptance is obtained as the ratio of the number of simulated signal events satisfying the event selection criteria in each reconstructed category over the total number of generated events. 
  The highest-order SM predicition for the sum of the \VBF and \VH contributions is also shown for comparison.  }
  \label{tab:BSMyields_VBF}

   
     \vspace{0.1cm}
  %\setlength{\tabcolsep}{1cm}
  {\renewcommand{\arraystretch}{1.5}
  \resizebox{\linewidth}{!}{


\begin{tabular}{l|c|cc|cc}

\hline\hline

 Reconstructed & Highest-order &   
 \multicolumn{2}{c|}{\progname{MadGraph5\_aMC@NLO}} &  
 
 \multicolumn{2}{c}{\progname{MadGraph5\_aMC@NLO}}\\
 
 event category & SM prediction                   &  
 \VBF+\STXSVHHad              & 
 \STXSVHLep               & 
 \VBF+\STXSVHHad  &
 \STXSVHLep  \\ 


 &    \VBF+\VH              &  
 (SM)  &  (SM) &
 \multicolumn{2}{c}{(\kSM = 1, | \kAVV | = 5)} \\ 
 \hline 

 
  
%$m_{4\ell}$-cut 	& 6.13 & 4.56 & 0.46 & 14.95 & 3.38 \\

\CatZeroJ 	& 0.54 & 0.27 & 0.13 & 0.39 & 0.74 \\

\CatOneJL 	& 0.74 & 0.53 & 0.03 & 0.83 & 0.09 \\

\CatOneJM &  0.87 & 0.57 & 0.03 & 1.17 & 0.17 \\
	
\CatOneJH & 0.37 & 0.21 & 0.03 & 1.29 & 0.42\\

\CatVBFLow & 2.29 & 2.15 & 0.03 & 4.75 & 0.22 \\

\CatVBFHigh	 & 0.23 & 0.23  & 0.00 & 3.11 & 0.05 \\

\CatVHHadLow & 0.59 & 0.43 & 0.01 & 1.44 & 0.06 \\
	
\CatVHHadHigh  & 0.21 & 0.15 & 0.01 & 1.84 & 0.08 \\

\CatVHLep 	& 0.27 & 0.004 & 0.20 & 0.02 & 1.54\\

\CatttH 	& 0.03 & 0.01 & 0.00 & 0.12 & 0.01 \\
\hline\hline
\end{tabular}
}}
\end{table*}







\end{document}

